Reflectance and fluorescence characteristics of PTFE coated with TPB at visible, UV, and VUV as a function of thickness

Polytetrafluoroethylene (PTFE) is an excellent diffuse reflector widely used in light collection systems for particle physics experiments. In noble element systems, it is often coated with tetraphenyl butadiene (TPB) to allow detection of vacuum ultraviolet scintillation light. In this work this dependence is investigated for PTFE coated with TPB in air for light of wavelengths of 200~nm, 260~nm, and 450~nm. The results show that TPB-coated PTFE has a reflectance of approximately 92\% for thicknesses ranging from 5~mm to 10~mm at 450~nm, with negligible variation as a function of thickness within this range. A cross-check of these results using an argon chamber supports the conclusion that the change in thickness from 5~mm to 10~mm does not affect significantly the light response at 128~nm. Our results indicate that pieces of TPB-coated PTFE thinner than the typical 10~mm can be used in particle physics detectors without compromising the light signal.

==> src/authors.tex <==
\collaboration{The NEXT Collaboration}
%
\author[11,a]{J.~Haefner,\note[a]{Corresponding author.}}
%
\author[11,a]{A.~Fahs,}
%
\author[11]{J.~Ho,}
%
\author[11]{C.~Stanford,}
%
\author[11]{R.~Guenette,}
%
\author[2]{C.~Adams,}
%
\author[11]{H.~Almaz\'an,}
%
\author[26]{V.~\'Alvarez,}
%
\author[24]{B.~Aparicio,}
%
\author[22]{A.I.~Aranburu,}
%
\author[7]{L.~Arazi,}
%
\author[20]{I.J.~Arnquist,}
%
\author[16]{S.~Ayet,}
%
\author[5]{C.D.R.~Azevedo,}
%
\author[2]{K.~Bailey,}
%
\author[26]{F.~Ballester,}
%
\author[21]{J.M.~Benlloch-Rodr\'{i}guez,}
%
\author[14]{F.I.G.M.~Borges,}
%
\author[11]{S.~Bounasser,}
%
\author[3]{N.~Byrnes,}
%
\author[19]{S.~C\'arcel,}
%
\author[19]{J.V.~Carri\'on,}
%
\author[27]{S.~Cebri\'an,}
%
\author[20]{E.~Church,}
%
\author[14]{C.A.N.~Conde,}
%
\author[11]{T.~Contreras,}
%
\author[21,9]{F.P.~Coss\'io,}
%
\author[4]{A.A.~Denisenko,}
%
\author[25]{G.~D\'iaz,}
%
\author[19]{J.~D\'iaz,}
%
\author[16]{T.~Dickel,}
%
\author[14]{J.~Escada,}
%
\author[26]{R.~Esteve,}
%
\author[7]{R.~Felkai,}
%
\author[13]{L.M.P.~Fernandes,}
%
\author[21,9]{P.~Ferrario,}
%
\author[5]{A.L.~Ferreira,}
%
\author[4]{F.W.~Foss,}
%
\author[13]{E.D.C.~Freitas,}
%
\author[22,9]{Z.~Freixa,}
%
\author[21]{J.~Generowicz,}
%
\author[8]{A.~Goldschmidt,}
%
\author[21,9,b]{J.J.~G\'omez-Cadenas\note[b]{ NEXT Co-spokesperson. },}
%
\author[21]{R.~Gonz\'alez,}
%
\author[25]{D.~Gonz\'alez-D\'iaz,}
%
\author[10]{R.M.~Guti\'errez,}
%
\author[2]{K.~Hafidi,}
%
\author[1]{J.~Hauptman,}
%
\author[13]{C.A.O.~Henriques,}
%
\author[25]{J.A.~Hernando~Morata,}
%
\author[21,23]{P.~Herrero-G\'omez,}
%
\author[26]{V.~Herrero,}
%
\author[7]{Y.~Ifergan,}
%
\author[3]{B.J.P.~Jones,}
%
\author[25]{M.~Kekic,}
%
\author[18]{L.~Labarga,}
%
\author[3]{A.~Laing,}
%
\author[6]{P.~Lebrun,}
%
\author[11]{D.~Lopez Gutierrez,}
%
\author[26]{N.~L\'opez-March,}
%
\author[10]{M.~Losada,}
%
\author[13]{R.D.P.~Mano,}
%
\author[19]{J.~Mart\'in-Albo,}
%
\author[19]{A.~Mart\'inez,}
%
\author[7]{G.~Mart\'inez-Lema,}
%
\author[21,19]{M.~Mart\'inez-Vara,}
%
\author[3]{A.D.~McDonald,}
%
\author[2]{Z.E.~Meziani,}
%
\author[3]{K.~Mistry,}
%
\author[21,9]{F.~Monrabal,}
%
\author[13]{C.M.B.~Monteiro,}
%
\author[26]{F.J.~Mora,}
%
\author[19]{J.~Mu\~noz Vidal,}
%
\author[3]{K.~Navarro,}
%
\author[19]{P.~Novella,}
%
\author[3,b,c]{D.R.~Nygren,}
%
\author[21]{E.~Oblak,}
%
\author[21]{M.~Odriozola-Gimeno,}
%
\author[25,19]{B.~Palmeiro,}
%
\author[6]{A.~Para,}
%
\author[12]{J.~P\'erez,}
%
\author[19]{M.~Querol,}
%
\author[3]{A.~Raymond,}
%
\author[7]{A.B.~Redwine,}
%
\author[25]{J.~Renner,}
%
\author[17]{L.~Ripoll,}
%
\author[21,9]{I.~Rivilla,}
%
\author[10]{Y.~Rodr\'iguez Garc\'ia,}
%
\author[26]{J.~Rodr\'iguez,}
%
\author[23]{C.~Rogero,}
%
\author[3]{L.~Rogers,}
%
\author[21,12]{B.~Romeo,}
%
\author[19]{C.~Romo-Luque,}
%
\author[14]{F.P.~Santos,}
%
\author[13]{J.M.F. dos~Santos,}
%
\author[7]{A.~Sim\'on,}
%
\author[19]{M.~Sorel,}
%
\author[13]{J.M.R.~Teixeira,}
%
\author[4]{P.~Thapa,}
%
\author[26]{J.F.~Toledo,}
%
\author[21]{J.~Torrent,}
%
\author[19]{A.~Us\'on,}
%
\author[5]{J.F.C.A.~Veloso,}
%
\author[4]{T.T.~Vuong,}
%
\author[15]{R.~Webb,}
%
\author[7,c]{R.~Weiss-Babai\note[c]{On leave from Soreq Nuclear Research Center, Yavneh, Israel. },}
%
\author[15,d]{J.T.~White\note[d]{Deceased. },}
%
\author[3]{K.~Woodruff,}
%
\author[19]{N.~Yahlali,}
%
\affiliation[1]{
Department of Physics and Astronomy, Iowa State University, Ames, IA 50011-3160, USA}
%
\affiliation[2]{
Argonne National Laboratory, Argonne, IL 60439, USA}
%
\affiliation[3]{
Department of Physics, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\affiliation[4]{
Department of Chemistry and Biochemistry, University of Texas at Arlington, Arlington, TX 76019, USA}
%
\affiliation[5]{
Institute of Nanostructures, Nanomodelling and Nanofabrication (i3N), Universidade de Aveiro, Campus de Santiago, Aveiro, 3810-193, Portugal}
%
\affiliation[6]{
Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
%
\affiliation[7]{
Nuclear Engineering Unit, Faculty of Engineering Sciences, Ben-Gurion University of the Negev, P.O.B. 653, Beer-Sheva, 8410501, Israel}
%
\affiliation[8]{
Lawrence Berkeley National Laboratory (LBNL), 1 Cyclotron Road, Berkeley, CA 94720, USA}
%
\affiliation[9]{
Ikerbasque (Basque Foundation for Science), Bilbao, E-48009, Spain}
%
\affiliation[10]{
Centro de Investigaci\'on en Ciencias B\'asicas y Aplicadas, Universidad Antonio Nari\~no, Sede Circunvalar, Carretera 3 Este No.\ 47 A-15, Bogot\'a, Colombia}
%
\affiliation[11]{
Department of Physics, Harvard University, Cambridge, MA 02138, USA}
%
\affiliation[12]{
Laboratorio Subterr\'aneo de Canfranc, Paseo de los Ayerbe s/n, Canfranc Estaci\'on, E-22880, Spain}
%
\affiliation[13]{
LIBPhys, Physics Department, University of Coimbra, Rua Larga, Coimbra, 3004-516, Portugal}
%
\affiliation[14]{
LIP, Department of Physics, University of Coimbra, Coimbra, 3004-516, Portugal}
%
\affiliation[15]{
Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843-4242, USA}
%
\affiliation[16]{
II. Physikalisches Institut, Justus-Liebig-Universitat Giessen, Giessen, Germany}
%
\affiliation[17]{
Escola Polit\`ecnica Superior, Universitat de Girona, Av.~Montilivi, s/n, Girona, E-17071, Spain}
%
\affiliation[18]{
Departamento de F\'isica Te\'orica, Universidad Aut\'onoma de Madrid, Campus de Cantoblanco, Madrid, E-28049, Spain}
%
\affiliation[19]{
Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Calle Catedr\'atico Jos\'e Beltr\'an, 2, Paterna, E-46980, Spain}
%
\affiliation[20]{
Pacific Northwest National Laboratory (PNNL), Richland, WA 99352, USA}
%
\affiliation[21]{
Donostia International Physics Center, BERC Basque Excellence Research Centre, Manuel de Lardizabal 4, San Sebasti\'an / Donostia, E-20018, Spain}
%
\affiliation[22]{
Department of Applied Chemistry, Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 3, San Sebasti\'an / Donostia, E-20018, Spain}
%
\affiliation[23]{
Centro de F\'isica de Materiales (CFM), CSIC \& Universidad del Pais Vasco (UPV/EHU), Manuel de Lardizabal 5, San Sebasti\'an / Donostia, E-20018, Spain}
%
\affiliation[24]{
Department of Organic Chemistry I, University of the Basque Country (UPV/EHU), Centro de Innovaci\'on en Qu\'imica Avanzada (ORFEO-CINQA), San Sebasti\'an / Donostia, E-20018, Spain}
%
\affiliation[25]{
Instituto Gallego de F\'isica de Altas Energ\'ias, Univ.\ de Santiago de Compostela, Campus sur, R\'ua Xos\'e Mar\'ia Su\'arez N\'u\~nez, s/n, Santiago de Compostela, E-15782, Spain}
%
\affiliation[26]{
Instituto de Instrumentaci\'on para Imagen Molecular (I3M), Centro Mixto CSIC - Universitat Polit\`ecnica de Val\`encia, Camino de Vera s/n, Valencia, E-46022, Spain}
%
\affiliation[27]{
Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias (CAPA), Universidad de Zaragoza, Calle Pedro Cerbuna, 12, Zaragoza, E-50009, Spain}
%
\emailAdd{jhaefner@g.harvard.edu}
\emailAdd{adam.fahs@mail.utoronto.ca}

==> src/authors_arxiv.tex <==
NEXT Collaboration: J. Haefner, A. Fahs, J. Ho, C. Stanford, R. Guenette, C. Adams, H. Almaz\'an, V. \'Alvarez, B. Aparicio, A.I. Aranburu, L. Arazi, I.J. Arnquist, S. Ayet, C.D.R. Azevedo, K. Bailey, F. Ballester, J.M. Benlloch-Rodr\'{i}guez, F.I.G.M. Borges, S. Bounasser, N. Byrnes, S. C\'arcel, J.V. Carri\'on, S. Cebri\'an, E. Church, C.A.N. Conde, T. Contreras, F.P. Coss\'io, A.A. Denisenko, G. D\'iaz, J. D\'iaz, T. Dickel, J. Escada, R. Esteve, R. Felkai, L.M.P. Fernandes, P. Ferrario, A.L. Ferreira, F.W. Foss, E.D.C. Freitas, Z. Freixa, J. Generowicz, A. Goldschmidt, J.J. G\'omez-Cadenas, R. Gonz\'alez, D. Gonz\'alez-D\'iaz, R.M. Guti\'errez, K. Hafidi, J. Hauptman, C.A.O. Henriques, J.A. Hernando~Morata, P. Herrero-G\'omez, V. Herrero, Y. Ifergan, B.J.P. Jones, M. Kekic, L. Labarga, A. Laing, P. Lebrun, D. Lopez Gutierrez, N. L\'opez-March, M. Losada, R.D.P. Mano, J. Mart\'in-Albo, A. Mart\'inez, G. Mart\'inez-Lema, M. Mart\'inez-Vara, A.D. McDonald, Z.E. Meziani, K. Mistry, F. Monrabal, C.M.B. Monteiro, F.J. Mora, J. Mu\~noz Vidal, K. Navarro, P. Novella, D.R. Nygren, E. Oblak, M. Odriozola-Gimeno, B. Palmeiro, A. Para, J. P\'erez, M. Querol, A. Raymond, A.B. Redwine, J. Renner, L. Ripoll, I. Rivilla, Y. Rodr\'iguez Garc\'ia, J. Rodr\'iguez, C. Rogero, L. Rogers, B. Romeo, C. Romo-Luque, F.P. Santos, J.M.F. dos Santos, A. Sim\'on, M. Sorel, J.M.R. Teixeira, P. Thapa, J.F. Toledo, J. Torrent, A. Us\'on, J.F.C.A. Veloso, T.T. Vuong, R. Webb, R. Weiss-Babai, J.T. White, K. Woodruff and N. Yahlali
